Cursed yet Satisfied Agents

In real life auctions, a widely observed phenomenon is the winner's curse -- the winner's high bid implies that the winner often over-estimates the value of the good for sale, resulting in an incurred negative utility. The seminal work of Eyster and Rabin [Econometrica'05] introduced a behavioral model aimed to explain this observed anomaly. We term agents who display this bias "cursed agents". We adopt their model in the interdependent value setting, and aim to devise mechanisms that prevent the cursed agents from obtaining negative utility. We design mechanisms that are cursed ex-post IC, that is, incentivize agents to bid their true signal even though they are cursed, while ensuring that the outcome is individually rational -- the price the agents pay is no more than the agents' true value. Since the agents might over-estimate the good's value, such mechanisms might require the seller to make positive transfers to the agents to prevent agents from over-paying. For revenue maximization, we give the optimal deterministic and anonymous mechanism. For welfare maximization, we require ex-post budget balance (EPBB), as positive transfers might lead to negative revenue. We propose a masking operation that takes any deterministic mechanism, and imposes that the seller would not make positive transfers, enforcing EPBB. We show that in typical settings, EPBB implies that the mechanism cannot make any positive transfers, implying that applying the masking operation on the fully efficient mechanism results in a socially optimal EPBB mechanism. This further implies that if the valuation function is the maximum of agents' signals, the optimal EPBB mechanism obtains zero welfare. In contrast, we show that for sum-concave valuations, which include weighted-sum valuations and l_p-norms, the welfare optimal EPBB mechanism obtains half of the optimal welfare as the number of agents grows large.

==> techniques.tex <==
\paragraph{Cursed Equilibrium and Ex-post solution concept} As discussed above, \citet{eyster2005cursed} suggest that the behavioral bias driving the winner's curse phenomenon is a result of agents' failure to estimate the contingency of other agents' actions on their signals. As a result, agents wrongly perceive their utility, which is modeled by taking a convex combination of $\chi$ times the expected utility when the other agents' signals are not associated with their actions and $1-\chi$ times the expected utility when they are ($\chi=0$ being a fully rational agent). Cursed agents play the equilibrium strategy  by correctly predicting the other agents' strategies, but based on a wrongly perceived utility function. We extend the cursed-equilibrium notion of \citet{eyster2005cursed} to a stronger solution concept of ex-post incentive compatibility according to the cursed utilities (\cepic). In a \cepic\ mechanism, truthful reporting strictly maximizes the cursed utility of agents given others reporting truthfully.  Similarly, cursed ex-post individual rationality (\cepir) is defined by cursed agents have non-negative ex-post utility based on their wrong reasoning. %, is defined as that the truthful reporting gives non-negative cursed utilities for them.
A key observation in \citet{eyster2005cursed} is that in auctions, the cursed agents act as if they are fully rational agents but with a modified valuation function $v_i^\chi$ parameterized by the cursedness parameter $\chi$. We refer to $v_i^\chi$ as the \textit{cursed valuation}. More on this in Section~\ref{sec:model}.

\citet{RoughgardenT16} provide a natural extension of Myerson's Lemma to ex-post implementation in interdependent value environments, where they show a mechanism is ex-post IC if and only if the allocation probability is monotone in each agent's signal, and the payment is defined by an extension of Myerson's payment identity. Their characterization combined with Eyster and Rabin's model implies a characterization on $\cepicir$ mechanisms for cursed agents, where $v_i$ is replaced with the cursed valuation $v_i^\chi$ in the payment identity (Proposition~\ref{thm:CEPICIR}). \citet{RoughgardenT16} also provided an analogue of virtual value theory for interdependent settings, which also extends to our setting (Proposition~\ref{thm:virtual-welfare}).

\paragraph{Achieving ex-post IR and implications}


Combining \epir\ and \cepicir\ constraints raises new challenges, as the first condition holds with respect to the \textit{real} valuation $v_i$, while the second condition holds with respect to the ``\textit{cursed}" valuation $v_i^\chi$. This implies that we cannot directly apply existing techniques. We first show that whenever we satisfy \epir\ when \cepic\ holds, this directly implies \cepir\ as well, so it's enough to focus on the former two conditions. Since we study deterministic mechanisms, the mechanisms' allocation rules can be represented by the threshold rules $t_i(\s_{-i})$, where agent $i$ wins in profile $\s$ whenever $s_i>t_i(\s_{-i})$. Given an threshold allocation rule, our only freedom in setting the payment is by setting the normalization term $p_i(0,\s_{-i})$ in the payment identity (Equation~\eqref{eq:payment identity}), as this is the only term that is not binding. We have two constraints on this term:
\begin{itemize}
	\item Since an agent $i$ should not have a negative utility when not receiving the item, $p_i(0,\s_{-i})$ cannot be positive.
	\item The binding part of the payment for a winning agent is the cursed valuation at the threshold of winning, i.e., $v_i^\chi(t_i(\s_{-i}),\s_{-i})$. The mechanism should compensate the agent when this is larger than the real value, otherwise the agent will receive a negative utility. The agent will receive the worst negative utility when her value is the the smallest possible winning value, i.e., at $v_i(t_i(\s_{-i}),\s_{-i})$. %Therefore, if $v_i^\chi(t_i(\s_{-i}),\s_{-i})>v_i(t_i(\s_{-i}),\s_{-i})
\end{itemize}
  Combining the two, we get that in order to satisfy $\epir$ while maximizing agents' payment, we need to set 
  %\begin{equation}
  $$
  p_i(0,\s_{-i}) =\min\{0, v_i(t_i(\s_{-i}),\s_{-i})-v_i^\chi(t_i(\s_{-i}),\s_{-i})\}%\label{eq_first_payid}
  $$
  %\end{equation}
  %$$p_i(0,\s_{-i}) = 
  %\begin{cases}\min\{0, v_i(t_i(\s_{-i}),\s_{-i})-v_i^\chi(t_i(\s_{-i}),\s_{-i})\} & \text{if } t_i(\s_{-i})<\bar{s}\\
  %0 & \text{if } t_i(\s_{-i})\ge\bar{s}
  %\end{cases}$$
  %$\bar{s}$ refers to the supremum of the signal space for each agent and $t_i(\s_{-i})\ge\bar{s}$ refers to the case that we do not allocate to agent $i$ whatever her signal is given $\s_{-i})$. In this case, no comp
  %\blue{whenever $t_i(\s_{-i})<\bar{s}$ with $\bar{s}$ the supremum of the signal space, meaning that we will allocate the item when agent $i$ has a signal higher than $t_i(\s_{-i})$. And in the case that we do not want to allocate the item to agent $i$ at $\s_{-i}$, i.e., $t_i(\s_{-i})\ge\bar{s}$, we set $p_i(0,\s_{-i})=0$.}
  Hence, given an allocation rule, we are able to give a binding payment identity. 

Plugging it back into the payment identity, we get that if an agent is allocated, she pays exactly the minimum between her valuation function and her cursed valuation at her threshold signal. This follows the intuition that in order to prevent the winner's curse, one needs to lower the payment to the actual value in order to prevent agents overpaying when winning. For a fixed signal profile, the winner's curse occurs whenever the agent has a higher expected value for the game not conditioning on the others' signals than conditioning on them. 
%\blue{the winner's curse occurs whenever the game gives the winner a higher expected value not conditioning on the others' signals than conditioning on them.} 
This implies that if for some $\chi > 0$, $v_i^\chi(t_i(\s_{-i}),\s_{-i})<v_i(t_i(\s_{-i}),\s_{-i})$, then for all $\chi'>0$, $v_i^{\chi'}(t_i(\s_{-i}),\s_{-i})<v_i(t_i(\s_{-i}),\s_{-i})$. This property is key in showing that for a fixed allocation rule, the revenue of an \epic\ and \cepicir\ mechanism decreases as $\chi$ increases, as it enables us coupling the different events. This claim is then used to show that the optimal revenue (and optimal welfare of an $\epbb$ mechanism) 
decreases as $\chi$ increases.


\begin{comment}
 for characterizing and analyzing the mechanisms, as the constraints contain two sets of valuation functions, and the existing techniques for the fully rational agents setting from~\cite{RoughgardenT16} no longer apply directly. 
To simplify the problem, we first show that \epir\  implies \cepir\ condition when \cepic\ holds so that we only need to focus on the \cepic\ and \epir\ constraints. 
Our characterization further relies on two critical observations. First, for any deterministic mechanism that satisfies the \cepic\ condition, the allocation rule is a threshold allocation rule, represented by $t_i(\s_{-i})$, so that agent $i$ wins the item when $s_i>t_i(\s_{-i})$. Second, the only freedom one has in designing the payment is by setting the initial payment of an agent ($p_i(0,\s_{-i})$ in Equation~\eqref{eq:payment identity}). 
Based on these two observations, it is sufficient for us to analyze the initial payment for an agent when the agent's signal is not higher than the threshold and when the agent's signal is higher than the threshold. For the former case, the agent receives no item and the initial payment only needs to be non-positive. For the latter case, the agent wins the item and has to pay the cursed valuation at the threshold signal ($v_i^\chi(t_i(\s_{-i}), \s_{-i})$) plus the initial payment. 
Meanwhile, the true valuation increases with the agent's  own signal. Therefore, \epir\ will be violated most when the agent's signal is exactly the threshold signal. Consequently, the optimal initial payment of the agent under a given threshold rule should be set to compensate exactly the overestimation of the item's value at the threshold signal.
 
 
Next, we focus on the impact of maintaining \epir\ on the optimal revenue and social welfare we can get for \cepicir\ mechanisms under different cursedness parameter $\chi$. Notice that the fully cursed valuation of the item is not necessary larger than the true value, and the compensation needed to maintain \epir\ may not necessarily increase with $\chi$. The key to draw the results that the optimal revenue and the social welfare decrease with $\chi$ is the observation derived from our above payment characterization that the winner actually pays the minimum of the true value and the cursed value of the item at the threshold signal, which decreases with $\chi$. 
 
 
 
 
 %We show that our solution concept (\cepicir\ and \epir) gives rise to an analogue of the payment identity of \epic\ mechanisms (Theorem~\ref{thm:CEPICIR}), but as opposed to the fully rational setting, we might need to set the constant term in the payment identity to be smaller than zero in order to maintain \epir. In other words, the mechanism might make positive transfers to compensate for the over-estimation of values due to the winner's curse. 

\end{comment}


\paragraph{Revenue maximization}
\citet{RoughgardenT16} show that revenue maximization for rational agents ($\chi=0$) has an analouge formulation to the optimal auction of \citet{myerson1981optimal}; 
i.e., revenue maximization can be modeled as \blue{separate} virtual value maximization problem \blue{for each signal profile $\s$, where} agents' signals are translated into conditional virutal valuations (conditioned on other agents' signals), and the item is allocated to the agent with the higher virtual valuation. However, this is not true for \epir\ mechanisms for cursed agents, as the normalization payment term $p_i(0,\s_{-i})$ cannot be factored into the virtual values formulation. This results in a more involved optimization task of a piece-wise function with an extra parameter, which is not easily separable. We use the \blue{anonymity assumption of the mechanisms} to simplify the problem to maximize the expected revenue extracted from a single agent. However, the allocation rule should still make sure at most a single agent is allocated at a time. We derive that the optimal solution satisfies the constraint that an agent is allocated only if her signal is the highest signal, resolving this issue. %The resulting allocation rule is to set the following allocation threshold:
% $$
% t_i^*(\s_{-i})=\mathrm{argmax}_{t\geq \max_{j\ne i} s_j} \min\{v_i^\chi(t,\s_{-i}), v_i(t,\s_{-i})\} - v_i^\chi(t,\s_{-i})F(t|\s_{-i}).
% $$


%\blue{However, the threshold allocation rule for a single agent is still bound by the threshold allocation rule via the constraint that only one item can be allocated at a time. We show that this constraint can be translated to an equivalent constraint for individual agents that their threshold signal should always greater than the highest signal of the other agents. Thus, the revenue maximization problem can be separated into revenue maximization problem for each single agent and each $\s_{-i}$, resulting in a simple solution form: the revenue optimal allocation rule is to allocate the item to agent $i$ whenever $s_i>t_i^*(\s_{-i})$ for 
%$$
%t_i^*(\s_{-i})=\mathrm{argmax}_{t\geq \max_{j\ne i} s_j} \min\{v_i^\chi(t,\s_{-i}), v_i(t,\s_{-i})\} - v_i^\chi(t,\s_{-i})F(t|\s_{-i}).
%$$
%}
%\blue{Juntao, I am confused regarding some of the text below.}

%For fully rational agents, it is well known that the revenue optimization problem can be modeled as a social welfare maximization problem with virtual valuations, which can be written as separable optimization problem for each signal profile $\s$. However, this is not true for \epir\ mechanisms for cursed agents, as the initial payment of an agent is non-zero and cannot be factorized into virtual values. To solve revenue maximization, using the symmetry assumption, we only need to  focus on maximizing the expected revenue extracted from one agent. For a single agent, the choice of the threshold allocation rule is independent of other agents' signals $\s_{-i}$. Similarly, the optimal initial payment of an agent given an threshold allocation rule is also fixed given $\s_{-i}$.  Therefore, we can decompose the overall revenue maximization problem into sub revenue maximization problems for each $\s_{-i}$, where we can derive analytical results. 

\paragraph{Welfare maximization} Welfare maximization is the most technically involved section of this paper. We now highlight the techniques used to obtain the results of this section.
%We require that the classic single-crossing condition holds for agents' valuation functions, which implies that an agent with a higher signal also has a higher valuation. We highlight the techniques we used to derive two main results in this part.  

Much of the results of this section rely on our characterization result showing that a mechanism is ex-post budget-balance (\epbb) if and only if the mechanism does not make positive transfers ($p_i(0,\s_{-i})=0,\forall i, \s_{-i}$). 
%First, \epbb\ implies no positive transfer. 
This characterization requires a natural cursedness-monotonicity condition: if an agent overestimates the value of the item at signal profile $\s$, then it still overestimates the value of the item when its signal is sufficiently large to win under $\s_{-i}$ and the others' signals decrease. This follows the intuition that a bidder might overestimate the value of the good for sale because her signal is higher than other signals, as shown in the wallet game example.  
To prove this characterization, we have the two following claims: 
\begin{enumerate}[(1)]
	\item For \epbb\ mechanisms, if $p_i(0,\s_{-i}) < 0$ (i.e., the mechanism uses positive transfers), then $t_i(\s_{-i})$ has to be equal to the highest signal in $\s_{-i}$. This lemma implies that if $p_i(\mathbf{0}) < 0$, then $t_i(\mathbf{0}_{-i})=0$, and thus agent $i$ also pays zero when winning.
	\item For \epbb\ mechanisms, if $p_i(0,\s_{-i}) < 0$, then whenever $i$'s signal is lower than the highest signal in $\s_{-i}$, the agent with the highest signal has to win (cannot not be a no allocation). This lemma implies that in this case, the winner might incur the winner's curse. 
\end{enumerate}


% Now we prove the main characterization using the above two lemmas as follows. Suppose there is a signal profile $\s$ such that agent $i$ receives a positive transfer from the mechanism (i.e., $p_i(0,\s_{-i})<0$).
% We iteratively transform the signal profile $\s$ until only one signal in $\s$ is non-zero --- at each iteration, we zero out the largest non-zero signal $j$ in $\s$. For the first round, we zero out agent $i$'s signal. After this zero-out operation, because of the second above lemma, agent $j$ with the highest signal in $\s_{-i}$ has to be the winner and because of the cursedness-monotonicity and the second lemma above, when we zero out the largest non-zero signal $j$ along with the second above claim to show that $p_i(0_{ij},\s_{-ij})<0$ as well. After finishing this iterative process, and ending up with a single $j\neq i$ such that $p_i(s_j, 0_{-j})<0$ and $s_j>0$, we use the first claim to show that for signal profile $\s=(s_j, 0_{-j})$, $p_j(\s)=0$ ($j$ wins but pays zero because all other agents' signals are zero and its threshold signal is also zero), and use the anonymity of the mechanism to show $p_{i'}(\s) < 0$ for $i'\neq j$. This violates the $\epbb$, which proves the characterization result. 


We then prove the main characterization as follows. %using the above two lemmas as follows. 
Suppose there is a signal profile $\s_{-i}$ such that agent $i$ receives positive transfers from the mechanism (i.e., $p_i(0,\s_{-i})<0$).  Then, consider a signal profile $\s:=(s_i,\s_{-i})$ where $s_i$ is the largest signal. We iteratively transform the  signal profile $\s$ until only a single signal in $\s$ is non-zero --- at each iteration, we zero out the largest non-zero signal  in $\s$. According to the second lemma above, after zeroing-out one signal, the agent with the next largest signal has to be the winner. Because of the cursedness-monotonicity, and since we start with agent $i$ who incurs the winner's curse (i.e., $p_i(0, \s_{-i})<0$), every winner during the process also incurs the winner's curse; thus, needs to be compensated. So in the $j$-th iteration, we get that $p_{(j)}(0,..,0,s_{(j+1)},...,s_{(n)})<0$ where $(j)$ refers to the $j$-th largest signal in $\s$. %is the along with the second above claim to show that $p_i(0_{ij},\s_{-ij})<0$ as well. 
At the end of this iterative process, we end up with $p_{(n-1)}(0,...,0,s_{(n)})<0$ and $s_{(n)}>0$. Since we consider anonymous mechanisms, this implies that $p_{(k)}(0,...,0,s_{(n)})<0,\forall k\ne n$. If we continue the iteration for one more step, we will get that $p_{(n)}(0,...,0,0)<0$ as well, and according to the first above lemma, we have $p_{(n)}(0,...,0,s_{(n)})=0$. This gives $\sum_i p_i(0,...,0,s_{(n)})<0$, which violates  \epbb\ and completes our proof of the characterization result. 






%To prove this characterization, we first show that having positive transfers for agent $i$ means $i$ wins whenever she has the highest signal. Otherwise, we construct a signal profile where no agent wins and the mechanism pays the agents, contradicting $\epbb$. We then show that whenever there are positive transfers for agent $i$ ($p_i(0,\s_{-i}) < 0$), then whenever $i$ is not the agent with the highest signal, the agent with the highest signal wins (again, by showing that otherwise we might make positive transfers while no agent is winning). We then use the two claims to prove the characterization as follows. Suppose there is a set of signals $\s_{-i}$ such that agent $i$ receives positive transfers from the mechanism (i.e., $p_i(0,\s_{-i})<0$).  We iteratively transform this set of signals where only a single signal in $\s_{-i}$ is non-zero --- at each iteration, we zero out the largest non-zero signal $j$ in $\s_{-i}$, and use the cursedness-monotonicity along with the second above claim to show that $p_i(0_{ij},\s_{-ij})<0$ as well. After finishing this iterative process, and ending up with a single $j\neq i$ such that $p_i(s_j, 0_{-j})<0$ and $s_j>0$, we use the first claim to show that for signal profile $\s=(s_j, 0_{-j})$, $p_j(\s)=0$ ($j$ wins but pays zero because all other agents' signals are zero and its threshold signal is also zero), and use the anonymity of the mechanism to show $p_{i'}(\s) < 0$ for $i'\neq j$. This violates the $\epbb$, which proves the characterization result. 
 
Recall that a masking operation of an allocation rule results in an allocation rule that allocates in a maximal subset of cases of the original allocation while guaranteeing no positive transfers. An implication of the above characterization is that the welfare-optimal \epbb\ mechanism is a masked mechanism. We show that in fact, the welfare-optimal \epbb\ mechanism is a masking of the optimal allocation rule, as using a different allocation rule either results in positive transfers, non-feasibility, or lower welfare. We term the welfare-optimal \epbb\ mechanism \textit{masked GVA} (masked generalized Vickrey auction).

The above characterization implies that for some functions, e.g., the $\max$ of agents signals, the welfare-optimal \epbb\ mechanism obtains 0 welfare. We introduce a fairly general valuation class, Concave-Sum valuations, for which we proved that the masked GVA mechanism gets at least half of the optimal unconstrained welfare as the number of agents grows large. The concave-sum valuation class contains functions of the form $v_i(\s) = \ell(g(s_i)+\sum_{j\neq i} h(s_j))$ where $\ell,g,h$ are increasing and $\ell$ is concave. As an example, setting $g,h$ to be linear functions, and $\ell$ to be the identity recovers the well-studied weighted-sum valuation class~~\citep{RoughgardenT16, EdenFFGK19, EdenFTZ21, myerson1981optimal}. The key to obtain the approximation guarantees is to find a probabilistic event that
\begin{enumerate}[(i)]
	\item happens with probability at least $1/2$ as the number of agents grow large, and 
	\item the expected welfare of the masked GVA mechanism conditioned on this event is higher than the expected unconditional optimal welfare.
\end{enumerate} 
Defining this probabilistic event, and proving the conditions hold for this event requires making subtle probabilistic claims, and is the most technically involved part of our paper.

For ease of exposition, consider the simple case where $v_i(\s)=\sum_i s_i$, and each signal's maximum value is 1. For this simple case, the probabilistic event boils down to having $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$. Applying the central limit theorem and using the fact that signals are sampled i.i.d., we get that this event happens with probability that goes to $1/2$ as the number of agents grows large, proving the (i) holds.  
  % (i) happens with a constant probability (1/2) when the number of agents grow large, (ii) the expected welfare of the masked GVA mechanism conditioned on this event is higher than the expected unconditional welfare.
% is higher conditioning on this event.  For ease of presentation, we now discuss the simple case where $v_i(\s)=\sum_j s_j$, and each signal's maximum value is 1. For this simple case, the probabilistic event boils down to having $\sum_j s_j\ge \E_\s[\sum_j s_j]+1$. Applying the central limit theorem and using the fact that signals are sampled i.i.d., we get that this event happens with probability that goes to $1/2$ as the number of agents grows large. 
To show (ii), we first show that whenever $\sum_j s_j\ge \E_\s[\sum_j s_j]+1$ happens, the agent does not overestimate the value of the item. This follows since the condition implies that $\sum_{j\neq i}s_j\geq \E_\s[\sum_{j\neq i} s_j]$, which implies the the cursed valuation of the winner is no larger than her true valuation. Therefore, the item will be allocated by the masked GVA. Next, we show that the expected highest valuation of among all agents conditioned on the event is no less than the unconditional expectation of the highest valuation. To obtain a rigorous proof, we re-construct the valuation function as a function of order statistics of all signals, and use the fact that for each order statistics, the conditional valuation first-order stochastic dominates its unconditional valuation.  

%the expected welfare of  the welfare-optimal \epbb\ mechanism conditioned on this condition is higher than the unconditional full efficiency. An analogy of this condition when the valuation is the sum of all signals is  $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$, where 1 represents the 
%supremum of a single signal. According to the central limit theorem, it will happen with 1/2 probability when the number of agents grow large. Next we need to show requirement (ii) also holds. We also divide the proof into two parts. First, we show that when $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$ happens, the winner will not overestimate the value of the item. This is where ``+1'' in the condition come into play. It guarantees that the sum of signals of all agents, excluding the winner (the agent with the highest signal) is still greater than its expectation. Thus, the cursed valuation of the winner is smaller than the corresponding true valuation and the masked generalized Vickrey auction will allocate the item to the agent with the highest signal as it won't incur  positive transfer. Second, we show that the expected highest valuation of among all agents conditioned on $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$ is no less than the unconditional expectation of the highest valuation. To obtain a rigorously proof, we re-construct the valuation function as a function of order statistics of all signals and use the fact that for each order statistics, the conditional version  first-order stochastic dominates its unconditional version. 


 %whenever a positive transfer is made to agent $i$ for a given signal profile $\s_{-i}$ (i.e., $p_i(0,\s_{-i})<0$) under \epbb, the threshold signal of agent $i$ to win the item has to be exactly the same as the highest signal in $\s_{-i}$ (i.e., cannot be larger than it). Second, we prove that in the same case, the threshold for agent $j$ who has the highest signal in $\s_{-i}$ is less than its own signal, i.e., whenever $s_i<s_j$ with the same $\s_{-ij}$, agent $j$ has to be allocated with the item. Equipped with these two results, we are able to prove the first main result   by constructing a counter example using induction. Suppose that there exists a signal profile $\s_{-i}$ that requires a positive transfer to agent $i$, i.e., $p_i(0,\s_{-i})<0$. Then, if we lower $s_i$ to zero, the item has to be allocated to agent $j$ and due to the cursedness-monotonicity and the symmetric setting, the initial payment of agent $j$'s should be negative as well, i.e., $p_j(s_j=0, s_i=0,\s_{-ij})<0$. By symmetry, we also have $p_i(s_j=0, s_i=0,\s_{-ij})<0$ for agent $i$.  By induction, we can iteratively lower the current highest signal to zero, while the initial payment of all agents with zero signal has to be negative. Finally, we will reach a signal profile with only one non-zero signal, while the sum of all agents' payments are equal to the sum of their initial payments, which are negative, violating \epbb. 

%With the first main result, it is easy to see that the welfare-optimal \epbb\ mechanism is the result of masking the generalized Vickrey auction, which always allocate the item to the agent with the highest valuation whenever no positive transfer is incurred. 

%Second, the welfare-optimal \epbb\ mechanism gets at least half of the full efficiency for concave-sum valuations when the number of agents grows large. The full efficiency is the expectation of the highest valuations among all agents. 

%The key to obtain this result is to find a subtle condition of the signal profile that satisfies (i) it happens with a constant probability (1/2) when the number of agents grow large, (ii) the expected welfare of  the welfare-optimal \epbb\ mechanism conditioned on this condition is higher than the unconditional full efficiency. An analogy of this condition when the valuation is the sum of all signals is  $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$, where 1 represents the 
%supremum of a single signal. According to the central limit theorem, it will happen with 1/2 probability when the number of agents grow large. Next we need to show requirement (ii) also holds. We also divide the proof into two parts. First, we show that when $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$ happens, the winner will not overestimate the value of the item. This is where ``+1'' in the condition come into play. It guarantees that the sum of signals of all agents, excluding the winner (the agent with the highest signal) is still greater than its expectation. Thus, the cursed valuation of the winner is smaller than the corresponding true valuation and the masked generalized Vickrey auction will allocate the item to the agent with the highest signal as it won't incur  positive transfer. Second, we show that the expected highest valuation of among all agents conditioned on $\sum_i s_i\ge \E_\s[\sum_i s_i]+1$ is no less than the unconditional expectation of the highest valuation. To obtain a rigorously proof, we re-construct the valuation function as a function of order statistics of all signals and use the fact that for each order statistics, the conditional version  first-order stochastic dominates its unconditional version. 

==> trashed.tex <==
	\begin{comment}
	
	\begin{lemma}
	Given valuation functions $\{v_i\}_{i\in [n]}$ that satisfy the single-crossing condition, then cursed valuation functions, $\{v_i^\chi\}_{i\in [n]}$, also satisfy the signal-crossing condition whenever signals $\s$ are sampled independently. 
	\end{lemma}
	\begin{proof}
	For any agents $i,j$ with $s_i>s_j$, we first have  $\E_{\tilde{\s}_{-i}}[v_i(s_i,\tilde{\s}_{-i})]=\int_{\tilde{\s}_{-i}}f(\tilde{\s}_{-i})v(s_i,\tilde{\s}_{-i})d\tilde{\s}_{-i}\ge \int_{\tilde{\s}_{-j}}f(\tilde{\s}_{-j})v(s_j,\tilde{\s}_{-j})d\tilde{\s}_{-j} = \E_{\tilde{\s}_{-j}}[v_j(s_j,\tilde{\s}_{-j})],$ because of the symmetry, independence of signals, and monotonicity of $v_{i}(\s)$ in $s_i$. Second, we have $v_i(\s)\ge v_j(\s)$ due to the single crossing condition. Therefore, $v_i^\chi(\s)=(1-\chi)v_i(\s)+\chi\E_{\tilde{s}_{-i}}[v_i(\tilde{s}_{-i},s)]\ge  (1-\chi)v_j(\s)+\chi\E_{{\tilde{s}_{-i}}}[x_j(\tilde{s}_{-j},s_j)]= v_j^\chi(\s)$.
	     
	\end{proof}
	
	\begin{corrolary}~\label{cor:gva-fully-efficient}
	    The GVA allocation rule with respect to $\chi$-cursed valuations is identical to the GVA allocation rule with respect the the true valuations, implying it is fully efficient. 
	%The GVA allocation rule for cursed valuation functions with parameter $\chi$ is monotone non-decreasing for any $\chi \ge 0$.
	\end{corrolary}
    
    \end{comment}


	\begin{comment}

	\begin{definition}[Generalized Myerson Auction (GMA)~\cite{RoughgardenT16}]
		\AE{Do we need it?}
	\end{definition}	We introduce the following definition:
	\begin{definition}[Critical-value and cursed critical value]
	The \textit{critical value} and cursed critical signal of agent $i$ at a set of signals $\s_{-i}$ are $c_i(\s_{-i})=v_i(t_i(\s_{-i}), \s_{-i})$ and $c_i^\chi(\s_{-i})=v_i^\chi(t_i(\s_{-i}), \s_{-i})$, respectively; that is, the valuation and cursed valuation at the critical bid. \label{def:critical-values}
	\end{definition}
	\end{comment}


	\begin{comment}
	\subsection{Assumptions}\label{sec:assumptions}
	
	When designing revenue optimal and approximate mechanisms, we use the standard assumptions of \citet{RoughgardenT16} (similar assumptions have been made throughout in the interdependent values literature~\cite{li2017approximation}, see \cite{RoughgardenT16} for detailed discussion and justification of these assumptions).
	
	%\begin{assumption}
	%	\label{ass_val_monotone}
	%	For any agent $i$, $v_i(\s)$ is non-decreasing in $s_j$ for any signal $s_j, j\in\N$. 
	%\end{assumption}
	
	\begin{assumption}
		\label{ass_signal_affiliation}
		Agents' signals satisfy affiliation, (e.g., roughly $\forall, i, j\in \N, \E[g(s_j)|s_i]$ in non-decreasing in $s_i$ for any non-decreasing function $g(\cdot)$.)
	\end{assumption}
	
	(Note: The \textbf{affiliation} condition refers to:
	\begin{quote}
		Intuitively, signals are affiliated when observing a subset of high signals makes it more likely that the remaining signals are also high. 
		Formally, for every pair of signal profiles $\s,\t$, it must hold that
		$$
		f(\s\wedge\t)f(\s\vee\t)\ge f(\s)f(\t),
		$$
		where $(\s\wedge\t)$ is the component-wise maximum, and $(\s\vee\t)$ is the component-wise minimum. Note that above inequality holds with equality for independent signals.
	\end{quote}
	Here $f(\cdot)$ is the density function. 
	)
	
	
	MISSING LOPOMO ASSUMPTION
	
	\end{comment}
	
	
	
	
	


\begin{theorem}
When the valuation function can be expressed in the form of  $v_i(\s)=l(g(s_i)+\sum_{j\ne i}h(s_j))$, where $g, h, l$ are strictly increasing, and $l$ is concave, and the bidders are fully cursed (i.e., $\chi=1$), then the masked Myerson mechanism (\MMyerson) maintains at least  $\frac{1}{2}$ of the optimal revenue one can get without the EP-IR constraint.
\end{theorem}


\begin{proof}
For the masked Myerson mechanism, we have $REV^\Mask(\s)=REV^\textsf{OPT}(\s)$ for $\s$ which satisfies $\bar{h}\ge \lambda+\frac{b}{n}$, as when $\bar{h}\ge\lambda+\frac{b}{n}$ holds, the masked Myerson mechanism has  exactly the same allocation rule and payment as those of the Myerson mechanism. When $\chi=1$, the auction degenerates to single-item independent private value auction, where $REV^\textsf{OPT}(\s)$ is non-decreasing in $s_i$ for all $i$ given any $\s_{-i}$. Therefore, we can prove the theorem similarly to the proof of Theorem~\ref{thm_masked_SW}.
% similarly, we have when $n\rightarrow+\infty$ 
% $$
% \E_s[REV^\Mask(\s)] \ge \frac{1}{2}\E_s[REV^{\textsf{OPT}}(\s)].
% $$

% Meanwhile, $REV^\textsf{OPT}(\s)$ is also non-decreasing in $s_{i^*}$ and $\bar{l}_{-i}$ as
% $$
% REV^\textsf{OPT}(\s)=
% \begin{cases}
% v^\chi(t_{i^*}(\s_{-i^*}), \s_{-i^*}) = 
% \end{cases}$$ is also 


% Therefore, when $n\rightarrow+\infty$, we have 
% \begin{align*}
% \E_s[REV^\Mask(\s)] \ge & \E_\s\left[REV^\textsf{OPT}(\s)\big|\bar{l}>\lambda+\frac{b}{n}\right]\cdot\Pr\left[\bar{l}>\lambda+\frac{b}{n}\right]\\
% \ge &  \E_\s\left[REV^\textsf{OPT}(\s)\right]\cdot\Pr\left[\bar{l}>\lambda+\frac{b}{n}\right]\\
% = & \frac{1}{2}\E_s[REV^{\textsf{OPT}}(\s)]
% \end{align*}

% \red{
% Note that the second inequality is because 
% \begin{align*}
% \E_\s\left[REV^\textsf{OPT}(\s)\big|\bar{l}>\lambda+\frac{b}{n}\right]     
% = &
% \sum_i \E_{\s_{-i}}\left[\E\left[p_i^\textsf{OPT}(\s)|l_i> \lambda+\frac{b}{n}-(n-1)\bar{l}_{-i}\right]\right] \\
% \end{align*}
% }


\end{proof}




\section{Socially optimal, C-EPIC-IR, EP-IR, EP-BB mechanism}

\begin{align*}
\max~& \E[\sum_i x_i(\s)v_i(\s)]\\
s.t.~~& \forall \s_{-i}, x_i(\s) \text{ is non-decreasing in } s_i\\
& \forall \s, i, p_i(\s) = x_i(\s)v_i^\chi(\s)-\int_{v_i^\chi(0,\s_{-i})}^{v_i^\chi(\s)}x_i((v_i^\chi)^{-1}(t|\s_{-i}), \s_{-i})dt - (x_i(0,\s_{-i})v_i^\chi(0,\s_{-i}) - p_i(0, \s_{-i})) \\
& \forall \s, i, x_i(\s)v_i(\s)-p_i(\s)\ge 0(\text{EP-IR})\\
& \forall \s, i, p_i(\s) \ge 0 (\text{EP-BB})
\end{align*}
$\Leftrightarrow$
\begin{align*}
\max~& \E[\sum_i x_i(\s)v_i(\s)]\\
s.t.~~& \forall \s_{-i}, x_i(\s) \text{ is non-decreasing in } s_i\\
& \forall \s, i, p_i(0,\s_{-i})\le x_i(\s)(v_i(\s)-v_i^\chi(\s))+\int_{v_i^\chi(0,\s_{-i})}^{v_i^\chi(\s)}x_i((v_i^\chi)^{-1}(t|\s_{-i}), \s_{-i})dt + x_i(0,\s_{-i})v_i^\chi(0,\s_{-i})\\
& \forall \s_{-i}, i, p_i(0,\s_{-i}) \ge 0
\end{align*}
$\Leftrightarrow$
\begin{align*}
\max~& \E[\sum_i x_i(\s)v_i(\s)]\\
s.t.~~& \forall \s_{-i}, x_i(\s) \text{ is non-decreasing in } s_i\\
& \forall \s, i, 0\le x_i(\s)(v_i(\s)-v_i^\chi(\s))+\int_{v_i^\chi(0,\s_{-i})}^{v_i^\chi(\s)}x_i((v_i^\chi)^{-1}(t|\s_{-i}), \s_{-i})dt + x_i(0,\s_{-i})v_i^\chi(0,\s_{-i})\\
\end{align*}

This is a linear optimization problem (at least when the signals are discrete.)

\section{Masked Myerson}
\label{sec:masked-myerson}



\AE{Move to appendix}	

	\subsection{optimal mechanisms}
	   
	
	
	
	\begin{proposition}
	Let $\mathcal{NC}^\textsf{Myerson}_{+}(\s_{i})=\{t|t\ge t_i^\textsf{Myerson}(\s_{-i}),t\in\mathcal{NC}(\s_{-i})\}$ and let $\mathcal{NC}^\textsf{Myerson}_{-}(\s_{i})=\{t|t\le t_i^\textsf{Myerson}(\s_{-i}),t\in\mathcal{NC}(\s_{-i})\}$.
	Let $\mathcal{T}(\s_{-i})$ be a set which contains=$\{\inf \mathcal{NC}^\textsf{Myerson}_{+}(\s_{-i})$ if $\mathcal{NC}^\textsf{Myerson}_{+}(\s_{-i})\ne \emptyset$, and contains $\sup\mathcal{NC}^\textsf{Myerson}_{+}(\s_{-i})\}$ if $\mathcal{NC}^\textsf{Myerson}_{+}(\s_{-i})\}\ne \emptyset$, and does not contain any other element. 
	The masked mechanism with the following threshold allocation rule is the revenue-optimal mechanism among deterministic, anonymous, \cepicir, \epir\ and $\epbb$ mechanisms:
	$$t_i^\Mask(\s_{-i})=
	\begin{cases}
	 t_i^\textsf{Myerson}(\s_{-i})\qquad & \text{if } t_i^\textsf{Myerson}(\s_{-i})\in\mathcal{NC}(\s_{-i}) \\
	 \text{argmax}_{t\in\mathcal{T}(\s_{-i})} \int_t^{\bar{s}}\phi_i^\chi(z,\s_{-i})dz  & \text{if } t_i^\textsf{Myerson}(\s_{-i})\notin \mathcal{NC}(\s_{-i}),\text{and } \mathcal{T}(\s_{-i}) \ne \emptyset\\
	 \bar{s}\qquad & \text{otherwise}
	\end{cases}.
	$$
	    \red{when the valuation function $v_i$ is continuous, satisfies cursedness-monotonicity and $v_i(\mathbf{0})=0$.} This mechanism degenerates to the masked Myerson mechanism when $v_i^\chi(\s)-v_i(\s)$ is non-increasing in $s_i$.
	\end{proposition}
	\begin{proof}
	
	By Theorem~\ref{thm:no-positive-transfers}, we note that the revenue optimal mechanism is a masked mechanism, where $p_i(0,\s_{-i})=0$ for all $i$ and $\s_{-i}$. Therefore, the expected revenue can be written as 
	\begin{align*}
	\E[REV(\s)] = & \E\left[\sum_i x_i(\s)\cdot \phi_i^\chi(\s)\right]\\    
	=& \sum_i \E_{\s_{-i}}\left[\E_{s_i}[x_i(\s)\cdot\phi_i^\chi(\s)]\right]\\
	=&\sum_i \E_{\s_{-i}}\left[\int_{t_i(\s_{-i})}^{\bar{s}}\phi_i^\chi(t,\s_{-i})dt\right]
	\end{align*}
	
	Due to the regularity condition, $\phi^\chi_i(t,\s_{-i})$ is non-decreasing in $t$. Thus, fixing $\s_{-i}$, $\int_{t_i(\s_{-i})}^{\bar{s}}\phi_i^\chi(t,\s_{-i})$ is a signal peak function with a minimal at $t_i^\textsf{Myerson}(\s_{-i})$, where $t_i^\textsf{Myerson}(\cdot)$ is the threshold allocation rule of the Myerson mechanism for cursed agents. Meanwhile, for any $\s_{-i}$ such that $t_i^{\textsf{Myerson}}(\s_{-i})\notin \mathcal{NC}(\s_{-i})$ and $\mathcal{NC}(\s_{-i})\neq \emptyset$, $\int_{t_i(\s_{-i})}^{\bar{s}}\phi_i^\chi(t,\s_{-i})$ is maximized at either $\sup\{t|t\in\mathcal{NC},t\le t_i^{\textsf{Myerson}}(\s_{-i})\}$ or $\inf\{t|t\in\mathcal{NC},t\le t_i^{\textsf{Myerson}}(\s_{-i})\}$. When $v_i^\chi(\s)-v_i(\s)$ is non-increasing in $s_i$ for any $\s_{-i}$. Then, for any $\s_{-i}$ such that $t_i^{\textsf{Myerson}}(\s_{-i})\notin \mathcal{NC}(\s_{-i})$ and $\mathcal{NC}(\s_{-i})\neq \emptyset$, $\{t|t\in\mathcal{NC},t\le t_i^{\textsf{Myerson}}(\s_{-i})\}=\emptyset$ and $\int_{t_i(\s_{-i})}^{\bar{s}}\phi_i^\chi(t,\s_{-i})$ is maximized at $\inf\{t|t\in\mathcal{NC},t\le t_i^{\textsf{Myerson}}(\s_{-i})\}$.
	For $\s_{-i}$ such that $\mathcal{NC}(\s_{-i})=\empty$ are masked mechanism never allocate the item, and $t_i(\s_{-i})=\bar{s}$.
	\end{proof}
	
	
	
	\begin{comment}
	\begin{corollary}
	For anonymous, deterministic, C-EPIC-IR, EP-IR mechanisms, if $\forall i, s_i\in[0,1]$ and the valuation function is 
	\begin{enumerate}
	    \item $v_i(\s) = \max_j\{s_j\}$, or
	    
	    \item a weighted function of $\s$,  
	\end{enumerate} 
	then a mechanism is EP-BB iff the mechanism is a masked mechanism.
	\end{corollary}
	    
	
	\begin{corollary}
	For $s_i\in[0,1]$ and valuation function $v_i(\s)=\max_j\{s_j\}$ or $v_i(\s)$ being a weighted sum of $\s$, 
	among all anonymous, deterministic, C-EPIC-IR, EP-IR and EP-BB mechanisms, the masked second price auction maximizes the social welfare, and the masked Myerson auction  maximizes the revenue if the signal distribution satisfies the regularity condition. 
	\end{corollary}
	\end{comment}
	
% 	\begin{theorem}
% 	For anonymous, deterministic, C-EPIC-IR, EP-IR mechanisms, when $\forall i, v_i(\s)=\max_k\{s_k\}$ and $s_i\in[0,1]$, a mechanism is EP-BB iff the mechanism has no compensation. 
% 	\end{theorem}
% 	\begin{proof}
% 	As the "if" direction is obvious, we prove the "only if" direction. 
% 	We prove by contradiction. Suppose for an EP-BB mechanism, there exists $\s_{-i}$ such that $p_i(0, \s_{-i})<0$. Based on Lemma~\ref{lem_EPBB_2}, for $j=\text{argmax}_{k\ne i}\{s_k\}$, and for any $s_i<s_{-i}^*$, we have $t_j(\s_{-j})<s_j$. Thus, we have for any $s_i<s_{-i}^*$, $p_j(0, \s_{-j})=\min\{0, v_j(t_j(\s_{-j}), \s_{-j})-v_j^\chi(t_j(\s_{-j}),\s_{-j}))\}<0$, where the inequality is due to the property of  $v_i(\s)=\max_{k}\{s_k\}$. Based on Lemma~\ref{lem_EPBB_1}, we have $t_j(\s_{-j})=\max_{k\ne j}\{s_k\}.$
	
% 	Applying above argument interactively for all agents, we have for any sufficiently small  $\epsilon$, satisfying $\epsilon\in(0, \min_{k\ne i}\{s_k\})$, \begin{align*}
% 	p_1(0,\epsilon,\frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon)
% 	= & v_1(t_1(\epsilon, \frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon),\epsilon, \frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon)-v_1^{\chi=1}(t_1(\epsilon, \frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon),\epsilon, \frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon)
% 	\\= & v_1(\epsilon,\epsilon, \frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon)-v_1^{\chi=1}(\epsilon,\epsilon, \frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon) < -1/2,
% 	\end{align*}and $p_1(\epsilon, \frac{1}{2}\epsilon,...,\frac{1}{2}\epsilon)=v_1(\epsilon, \frac{1}{2}\epsilon,...,\frac{1}{2}\epsilon)=\epsilon.$ And thus, $REV(\epsilon,\frac{1}{2}\epsilon,..., \frac{1}{2}\epsilon) = \sum_k p_k(\s) = v_1(\epsilon, \frac{1}{2}\epsilon,...,\frac{1}{2}\epsilon) + \sum_{k\ge 2} p_k(0, \epsilon, \frac{1}{2}\epsilon,...,\frac{1}{2}\epsilon)<\epsilon+(n-1)\frac{1}{2}<0$, which violates the EP-BB property.
% 	\end{proof}
	
	
% 	\begin{theorem}
% 	For two-agent case, for anonymous, deterministic, C-EPIC-IR, EP-IR mechanisms, when the curse $v_i^\chi(\s)-v_i(\s)$ is non-decreasing in $s_i$ for any $\s_{-i}$ and $\lim_{t\rightarrow 0}v_i(t,t)=0$, a mechanism is EP-BB iff the mechanism has no compensation. 
% 	\end{theorem}
% 	\begin{proof}
% 	As the "if" direction is obvious, we prove the "only if" direction. 
% 	We prove by contradiction. Suppose for an EP-BB mechanism, there exists $s_j$ such that $p_i(0, s_j)<0$. Based on Lemma~\ref{lem_EPBB_1}, we have $t_i(s_j)=s_j$. Meanwhile,
% 	for a sufficiently small $\epsilon$, satisfying $0<\epsilon<s_j$, we have $v_j(\epsilon, \epsilon)-v_i^\chi(\epsilon,\epsilon)<0$, and as we assume $v_j^\chi(s_j, s_i)-v_j(s_j, s_i)$ is non-deceasing in $s_j$  for any $s_i$, we have $v_j(t_j(\epsilon), \epsilon)-v_j^\chi(t_j(\epsilon),\epsilon)<0$ for any $t_j(\epsilon)<1$. Based on Lemma~\ref{lem_EPBB_2}, and $\epsilon<s_j$, we have $t_j(\epsilon)<s_j$, and thus, $p_j(0, \epsilon)=\min\{0, v_j(t_j(\epsilon), \epsilon)-v_j^\chi(t_j(\epsilon),\epsilon))\}<0$. Therefore, based on Lemma~\ref{lem_EPBB_1}, we have $t_j(\epsilon)=\epsilon.$
	
% 	Therefore, we have 
% 	\begin{align*}
% 	    REV(\epsilon, s_j)= & p_i(\epsilon,s_j)+p_j(s_j, \epsilon)\\
% 	    = & p_i(0, s_j)+v_j(\epsilon, \epsilon)
% 	    <0,
% 	\end{align*}
% 	which violates the EP-BB property. Note that the last inequality is due to $\lim_{t\rightarrow 0}, v_j(t,t)=0.$
% 	\end{proof}


%\input{behavioral_model_new}
